Level sets of asymptotic mean of digits function for 4-adic representation of real number

We study topological, metric and fractal properties of the level sets $$S_{\theta}=\{x:r(x)=\theta\}$$ of the function $r$ of asymptotic mean of digits of a number $x\in[0;1]$ in its $4$-adic representation, $$r(x)=\lim\limits_{n\to\infty}\frac{1}{n}\sum\limits^{n}_{i=1}\alpha_i(x)$$ if the asymptotic frequency $\nu_j(x)$ of at least one digit does not exist, were $$ \nu_j(x)=\lim_{n\to\infty}n^{-1}#\{k: \alpha_k(x)=j, k\leqslant n\}, \:\: j=0,1,2,3. $$

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{2}

